Computing Optimal Control of Cascading Failure in DC Networks

We consider discrete-time dynamics, for cascading failure in DC networks, whose map is composition of failure rule with control actions. Supply-demand at the nodes is monotonically non-increasing under admissible control. Under the failure rule, a link is removed permanently if its flow exceeds capacity constraints. We consider finite horizon optimal control to steer the network from an arbitrary initial state, defined in terms of active link set and supply-demand at the nodes, to a feasible state, i.e., a state which is invariant under the failure rule. There is no running cost and the reward associated with a feasible terminal state is the associated cumulative supply-demand. We propose two approaches for computing optimal control. The first approach, geared towards tree reducible networks, decomposes the global problem into a system of coupled local problems, which can be solved to optimality in two iterations. When restricted to the class of one-shot control actions, the optimal solutions to the local problems possess a piecewise affine property, which facilitates analytical solution. The second approach computes optimal control by searching over the reachable set, which is shown to admit an equivalent finite representation by aggregation of control actions leading to the same reachable active link set. An algorithmic procedure to construct this representation is provided by leveraging and extending tools for arrangement of hyperplanes and polytopes. Illustrative simulations, including showing the effectiveness of a projection-based approximation algorithm, are also presented.

==> complexity.tex <==
\section{Complexity Analysis}
\label{sec:complexity-analysis}

This section includes discussion on the complexity of the optimal control problem and the relevant algorithms, as well as the extension to more general problem settings. A connected network \( \mathcal{G} = ( \mathcal{V}, \mathcal{E}) \)  is considered without loss of generality. If the network consists of multiple connected components, the same analysis can be applied on each component. In addition, we assume \( d := | \mathcal{V}_{l}| -1 \) to be a constant. 

\subsection{Complexity of Optimal Control of Cascading Failure}
\label{sec:problem-complexity} 

For a connected network \( \mathcal{G}= ( \mathcal{V}, \mathcal{E}) \), an initial supply demand vector \( p \) and a time constant \( N \), we define the \emph{complexity}, denoted by \( \kappa(\mathcal{E}, p, N) \), of the optimal control problem \eqref{eq:control-formulation-new} to be the number of possible topology sequences that can occur in \eqref{eq:cascade-dynamics} under all possible controls \( u\in \mathcal{D}( \mathcal{E}, p, N) \) (cf. \eqref{eq:feasible-set-def}). The rationale of the definition is as follows. One one hand, Remark~\ref{rem:aggregation-is-decomposition} implies in order to solve  \eqref{eq:control-formulation-new}, it is sufficient to solve \( \kappa(\mathcal{E}, p, N) \) number of linear programs. On the other hand, for a general network, due to non-monotonicity of power flow \cite{Ba.Savla:TCNS16, Ba.Savla.CDC16}, the only way to determine an ordering, in terms of residual load, between two topology sequences is through direct computation. Therefore, in principle all the \( \kappa(\mathcal{E}, p, N) \) topology sequences need to be considered in order to solve \eqref{eq:control-formulation-new} exactly. 

Consider the optimal control problem for a tuple \( ( \mathcal{E}, p, N) \). For an arbitrary aggregated state \( ( \mathcal{E}', P') \) (cf.  \eqref{eq:cascade-dynamics-aggregated-new}-\eqref{eq:partition-def}) and a link \( i\in \mathcal{E}' \), if \( \setdef{u\in \real^{ \mathcal{V}}}{ f_{i}( \mathcal{E}', u) < -c_{i}} \cap U( \mathcal{E}', P') \neq \emptyset \) (or  \( \setdef{u\in \real^{ \mathcal{V}}}{ f_{i}( \mathcal{E}', u) > c_{i}} \cap U( \mathcal{E}', P') \neq \emptyset \), respectively), then we call the constraint \( f_{i}( \mathcal{E}, u) \ge -c_{i} \) (or \( f_{i}( \mathcal{E}, u) \le c_{i} \), respectively) an \emph{intersecting constraint} and link \( i \) an infeasible link (in both case). 
Let \( n( \mathcal{E}, p, N) \) be the maximal number of intersecting constraints over all aggregated states. It is clear that \( n( \mathcal{E}, p, N) \) is upper bounded by twice of the maximal number of infeasible links over all aggregated states. We then have the following result on \( \kappa( \mathcal{E}, p, N) \). 

\begin{proposition}
\label{prop:complexity}
For a connected network \( \mathcal{G}= ( \mathcal{V}, \mathcal{E}) \), an initial supply demand vector \( p \) and a time constant \( N \),  \( \kappa( \mathcal{E}, p, N)= O(n^{d(N-1)}) \), where \( n := n ( \mathcal{E}, p, N) \) is the maximal number of intersecting constraints, \( d := | \mathcal{V}_{l}(p)| -1 \), \( |\mathcal{V}_{l}(p)| \) is the number of non-transmission nodes in \( \mathcal{G}\). 
%Furthermore, there exists a choice of \(  \mathcal{G}= ( \mathcal{V}, \mathcal{E})  \), \( p \) and \( N \) such that the bound is tight, that is, \( \kappa( \mathcal{E}, p, N)= \Theta(n^{d(N-1)}) \). In these bounds the constant of proportionality depends on \( d \). 
\end{proposition}
\begin{proof}
We first show that \( \kappa( \mathcal{E}, p, N)= O(n^{d(N-1)})  \). It is clear that from the definition in \eqref{eq:partition-def}, at an aggregated state \( (\mathcal{E}', P) \), the number of possible topologies at the next stage is no larger than \( | \mathbb{U}( \mathcal{E}, P) | \). From Section~\ref{subsec:arrangement}, we know that \( \mathbb{U}( \mathcal{E}, P) \) contains a subset of cells, the ones within \( U( \mathcal{E}, P) \), of the associated arrangement, that is, the arrangement of the hyperplanes associated with intersecting capacity constraints at \( ( \mathcal{E}, P) \). According to \cite[Chapter 24]{toth2004handbook}, \( | \mathbb{U}( \mathcal{E}, P) |  = O(n^{d}) \).
%\( | \mathbb{U}( \mathcal{E}, P) |  \) is upper bounded by \( \sum_{i= 0}^{d} {\hat{n} \choose i} \). For \( d \le \hat{n}/2 \), \(  \sum_{i= 0}^{d} {\hat{n} \choose i} \le \frac{\hat{n}-d}{\hat{n}-2d}  {\hat{n} \choose d} = O(\hat{n}^{d})  \). For  \( d > \hat{n}/2 \), \( \sum_{i= 0}^{d} {\hat{n} \choose i} \le 2^{\hat{n}} = O(4^{d})  \) \footnote{\({n \choose k}\) is defined to be 0 for \( n < k \).}. It is then clear that \( | \mathbb{U}( \mathcal{E}, P) |  = O(n^{d}) \) for all aggregated state \( ( \mathcal{E}, P) \). 
In other words, the branching factor of the aggregated search tree is \( O(n^{d}) \). Nevertheless, the additional constraints on the control at \( t= N-1 \), as commented in Remark~\ref{rem:additional-check}, implies that \( |U( \mathcal{E}, P)| = 1 \) for all aggregated state \( ( \mathcal{E}, P) \) at \( t= N-1 \). It is equivalent to consider the depth of the search tree to be \( N-1 \). Therefore, the total number of topology sequences is \( \kappa( \mathcal{E}, p, N)= O(n^{d(N-1)}) \). 
%Furthermore, the network in Fig.~\ref{fig:net-1s2d}, with \( N=2 \), provides an example to show that the bound can be tight. In this example, \( n=3 \), \(d = 2 \) and the number of topology sequences is \( \sum_{i=0}^{3} {3 \choose i} = 7 \). 
\end{proof}

\subsection{Time complexity of the solution methods}
\label{sec:running-time}

\begin{table}[htbp]
   \centering
      \caption{Comparison of time complexity of several algorithms.  \label{tab:complexity}}
   \begin{threeparttable}
   \begin{tabular}{lcc} % Column formatting, @{} suppresses leading/trailing space
      \toprule
      & Method & Time Complexity  \\
      \midrule
      %\multirow{3}{*}{General networks \( \mathcal{G} = ( \mathcal{V}, \mathcal{E}) \) }
      	   & Value iteration &   \( O\left(N2^{| \mathcal{E}|} n_{0}^{2d} T \right) \)  \\
            & Search with discretization & \( O\left(n_{0}^{d N} T \right) \) \\
                & Aggregated search with arrangement   & \( O\left( n^{dN} + n^{d(N-1)}  | \mathcal{V}|^{2} \right) \) \\
%     {Tree reducible networks}
             & Two iterations algorithm  &  \( O\left( | \mathcal{V}|^{2}\tilde{n}^{N-1} + | \mathcal{V}_{T}|  n_{0}^{ \hat{d} N}\right) \)  \\
      \bottomrule
   \end{tabular}
     \begin{tablenotes}
      {\scriptsize
      \item \( n_{0} \): number of discretized grid points along one dimension; 
      \item \( n = n( \mathcal{E}, p^{0}, N) \); 
      \item \( T \): time complexity for evaluating \( f( \mathcal{E}', p') \) at a given state \( ( \mathcal{E}', p') \);  
      \item \( \hat{d} \) is the maximal degree in the reduced tree;
      \item \( \tilde{n} = \max_{i\in \mathcal{E}_{T}} n( \mathcal{E}_{i}, a_{i}, N) \).
      }
    \end{tablenotes}
     \end{threeparttable}
\end{table}

Table~\ref{tab:complexity} shows the time complexities of solving the optimal control problem for a connected network \( \mathcal{G}= ( \mathcal{V}, \mathcal{E}) \) with initial supply-demand vector \( p^{0} \) by using different methods. In all these methods,  discretization, whenever used, is assumed to produce same number, denoted by \( n_{0} \), of grid points on every dimension, and \( T \) is used to denote the time to evaluate the value of \( f( \mathcal{E}', p') \) at a given state \( ( \mathcal{E}', p') \). The algorithms considered are as follows: 
\begin{enumerate}[(I)]
\item Value iteration: The state space is considered to be \( 2^{ \mathcal{E}} \times \mathcal{B}_{ \mathcal{E}} \). As \( \mathcal{B}_{ \mathcal{E}} \) is a linear subspace of dimension \( d \), the number of grid points for the state space is \( 2^{| \mathcal{E}|} n_{0}^{d} \). At each grid point \( ( \mathcal{E}', p') \) , computing the state transition requires evaluating function value \( f( \mathcal{E}', u) \) for all \( u\in U( \mathcal{E}', p') \). It takes \( O(n_{0}^{d} T) \). Therefore, the overall time for \( N \) time steps is \( O(N2^{| \mathcal{E}|} n_{0}^{2d} T ) \). 
\item Search with discretization: The control space \( U( \mathcal{E}', p')  \) for state \( ( \mathcal{E}', p') \) at each time step is discretized by \( n_{0}^{d} \) number of grid points. It is the branching factor of the search tree of depth equal to \( N \). Hence the total number of nodes in the tree is \( O(n_{0}^{dN}) \). In addition, computing flow and hence time \( T \) is required for state transition to each node. Therefore, the overall time complexity is \( O( n_{0}^{dN} T) \). It can be seen that the search method is more efficient than the value iteration if \( | \mathcal{E} | \ge d N \lg_{2} n_{0} \).
\item Aggregated search with arrangement: the proof of proposition \ref{prop:complexity} implies that the number of nodes in the aggregated tree is \( O(n^{d(N-1)}) \). At an aggregated state \( ( \mathcal{E}', P') \), Remark~\ref{rem:arrangement-construction} implies that \( \mathbb{U}( \mathcal{E}, P) \) can be computed in time \( O( n^{d}) \) through constructing the associated arrangements by using the incremental algorithm in Section~\ref{subsec:arrangement}. The overall time for constructing the aggregated search tree is \( O( n^{d(N-1)}) \). In addition, every node \( (\mathcal{E}', P') \) needs to conduct two computational tasks. The first task is to update the pseudo-inverse of Laplacian matrix according to the formula in \cite{ba2018elements}. This takes \( O(| \mathcal{V}|^{2}) \). The second task is to compute \( \cube{P}' \) using Proposition~\ref{prop:sweep-case-1} and Proposition~\ref{prop:top-facet-boundary-ridge}. Its time complexity is determined by the time complexity of a single sweep operation. The latter is bounded by the number of faces in \( P'\) and hence is \( O( n^{d}) \). Therefore, the overall time complexity for the aggregated tree search is \( O\left( n^{dN} + n^{d(N-1)}  | \mathcal{V}|^{2} \right) \). 
\item Two iteration algorithm: it works only for tree reducible network. Let the reduced tree be \( \mathcal{T} = ( \mathcal{V}_{T}, \mathcal{E}_{T}) \). The time complexity of the algorithm consists of two parts: computing \( \Drelone_{i} \) for all \( i\in \mathcal{E}_{T} \) and solving \eqref{opt:tree-dp-value-iteration} through discretization for all \( i\in \mathcal{V}_{T} \). This first part amount to constructing the aggregated search tree for a network that contains a single supply demand pair. Since the sweep operation in one dimensional space takes constant time, the above analysis implies that it takes time \( O\left( | \mathcal{V}_{i}|\tilde{n}^{N-1} \right) \) to compute \( \Drelone_{i} \) for \( \mathcal{G}_{i} = ( \mathcal{V}_{i}, \mathcal{E}_{i}) \), where \( \tilde{n} = \max_{i\in \mathcal{E}_{T}} n( \mathcal{E}_{i}, a_{i}, N) \) as defined in Section~\ref{sec:problem-complexity} and \( a_{i} \) is as shown in \eqref{eq:Drel-def}. It is straightforward to see that \( n( \mathcal{E}_{i}, a_{i}, N) \) is much smaller than \( n( \mathcal{E}, p, N) \) for all \( i\in \mathcal{E}_{T} \). Hence the total time for computing \( \Drelone_{i} \) all \( i\in \mathcal{E}_{T} \) is \( O( |\mathcal{V}|^{2}\tilde{n}^{N-1}  ) \), since in most cases \( \sum_{i\in \mathcal{E}_{T}} | \mathcal{V}_{i}|^{2}  \) is smaller than \( | \mathcal{V} |^{2} \). The second part is to solve sub-problems \eqref{opt:tree-dp-value-iteration} of a dimension no larger than \( N \hat{d} \), where \( \hat{d} \) is the maximal node degree of the reduced tree. Using the same discretization parameter \( n_{0} \), a single subproblem takes time \( O( n_{0}^{ \hat{d} N }) \) and the total time complexity of the recursive procedure is the summation of these subproblems over all nodes in \(\mathcal{T}\), that is, \( O\left( | \mathcal{V}_{T}|  n_{0}^{ \hat{d} N}\right) \). Therefore, the overall time complexity for the algorithm is  \( O\left( | \mathcal{V}|^{2}\tilde{n}^{N-1} + | \mathcal{V}_{T}|  n_{0}^{ \hat{d} N}\right) \).
%\item Algorithm \ref{alg:two-iterations}: assume \( \Dconstantrelone_{i} \), \( i\in \mathcal{E}_{T} \),  is known and satisfies the conditions in Proposition~\ref{prop:star-net-invariance}. Each node \( i\in \mathcal{V}_{T} \) in the reduced tree computes the value of top point and receives a solution of \( u_{i} \) and \( z_{i} \). It is straightforward that the overall time complexity is \( O( | \mathcal{V}_{T}|) \). 
\end{enumerate}

\begin{remark}
%\begin{enumerate}[(i)]
% \item In spite of the exponential time complexity (with respect to \( N \) and \( d \)), \kscomment{the aggregated tree search algorithm is optimal for general networks, in the same sense that the underlying algorithm for constructing the arrangements is optimal for general positioned hyperplanes}. The huge complexity can be attributed to the well known non-monotonicity of power flow in DC networks. Each path of the search tree corresponds to a possible topology sequence in the cascading failure dynamics. Due to non-monotonicity of power flow, in general, the only way to determine an ordering, in terms of residual load, between two topology sequences is through direct computation. Therefore, an optimal algorithm has to explore every path in the tree.
%
%Hence, in order to find the optimal load shedding policy, one has to construct and compute the value of each path at least once. 
%\kscomment{Provide an example, possibly a triangular network, to show that every path can be an optimal solution for proper weighs and capacities.}
%\item 
The time complexity for aggregated tree search may not be tight due to several reasons:
\begin{itemize} \ksmargin{clarify what does this mean}
\item The arrangement problem at a network state could be \kscomment{highly degenerated}, that is, two hyperplanes do not necessarily intersect and more than \( d \) hyperplanes can intersect at a vertex, in which case the corresponding branching factor is much smaller than \( n^{d}  \).
\item When the network gets disconnected due to link failures, \kscomment{the arrangement problem is solved for each connected component independently.} \ksmargin{correct?} Therefore, an accurate estimate of $d$ is related to the number of non-transmission nodes in a component, as opposed to the entire network. Since the number of connected components is non-decreasing along a path in the search tree, the pertinent value of $d$ may be much less than $|\mc V_l|-1$ away from the initial state $(\mc E^0,\{p^0\})$. 
\item As shown in Section~\ref{sec:algorithm-section}, lower and upper bounds at each aggregated state can be used to prune the aggregated search tree. This avoids searching through the entire aggregated state space without compromising the performance, and therefore improves the efficiency of the aggregated tree search algorithm. 
\end{itemize}
%Knowing that any practical network can contain a great number of generators and load buses, we must emphasis that the algorithm can perform much better in practice than the upper bound in previous paragraphs. 
%\sout{Finally, when dealing with practical problem, the algorithm provides the possibility for parallel computing and early termination. One can conveniently distribute the computation of different branches of the search tree to different processors. At the same time, a feasible solution with performance guarantee would be returned by the algorithm whenever it is terminated.} 
%\end{enumerate}
\end{remark}










==> opt-const-control.tex <==
\subsection{Optimal Constant Control Action for Tree Reducible Networks}
\label{sec:tree-reducible-constant-control}
Lemma~\ref{lem:meta-star-net}, Proposition~\ref{prop:star-net-invariance-ext} and Proposition~\ref{prop:star-net-invariance} can be used in the two iteration algorithm proposed in Section~\ref{sec:tree-reducible-net} to obtain an optimal load shedding control action within the class of constant control actions (cf. Definition~\ref{prop:para-net-opt-control}) for tree reducible networks. 
We provide the explicit algorithm in Algorithm~\ref{alg:two-iterations} for the case when the conditions in Proposition~\ref{prop:star-net-invariance} are satisfied. The algorithm for the general case can be extrapolated from this straightforwardly. With Remark~\ref{rem:correspondence} showing the correspondence between \eqref{opt:tree-dp-value-iteration} and \eqref{opt:lp-meta-star}, we use the following additional notation in Algorithm~\ref{alg:two-iterations}. Let \( \tau_{i} = (\tau_{i}^{1}, \tau_{i}^{2}) \) be the top point and \( [z_{i}^{l}, z_{i}^{u}] := \mathcal{Z}_{i} \) be the domain of function \( g_{i}(z) \) for all \( i\in \mathcal{V} \); the domain and the top point of function \( \sdsign_{i} z_{i} \) are \( \cube{p_{i}^{0}} \) and  \( (p_{i}^{0}, |p_{i}^{0}|) \), respectively. For a real number \( x \), let \( [x]^{+}:= \max\{x, 0\} \)  and \( [x]^{-}:= \min\{x, 0\} \). Hence,  \( \cube{p_{i}^{0}} \equiv \left[ [p_{i}^{0}]^{-}, [p_{i}^{0}]^{+} \right] \). Furthermore, let \( q_{i}>0 \) be the maximal value of \( \Drelone_{i} \) for the case of constant control for all \( i\in \mathcal{E}_{T} \). Remark~\ref{rem:d-rel-set} implies that \( -q_{i} \) is the minimal value of \( \Drelone_{i} \). 
%
%\begin{definition}[Constant Control Action]
%\label{def:constant-control}
%A \( N \) stage \qbcomment{feasible} control action $u \in \mc D$ is called constant if $u^t=u^{0}$ for all $t = 1, \ldots, N-1$. Let the set of feasible constant control actions be denoted by $\Dconstant$.
%\end{definition}
%
%Consider a reduced tree \( \mathcal{T} = ( \mathcal{V}, \mathcal{E}) \) with initial supply demand vector \( p^{0} \) and a constant control \( u \in \Dconstant \). 
%\sout{Under a $u \in \Dconstant$, all the load shedding is performed at $t=0$. However, $(\mc E^1,p^1)$ does not necessarily belong to $\mc S$, i.e., link failures could occur at $t \geq 1$. Nevertheless, $(\mc E^{N-1},p^{N-1})$ is guaranteed to be in $\mc S$ by definition of \( \Dconstant \). }
%Following the definition in \eqref{eq:Drel-def} and \eqref{eq:Si-def}, for all \( i\in \mathcal{E} \), let $\Dconstantrelone_{i}$ and $\Dconstantreltwo_{i}$ be the subsets of $\Drelone_{i}$ and $\Dreltwo_{i}$, respectively, corresponding to constant control actions.  Let \( \Dconstantrelone_{0} := \{ \zerobf \} \). Since each control action in $\Dconstantrelone$ and $\Dconstantreltwo$ can expressed in terms of only one scalar, irrespective of $N$, we consider  $\Dconstantrelone$ and $\Dconstantreltwo$ to be subsets of $\real$ for simplicity in presentation. It is straightforward to check that \( \Dconstantreltwo_{i} = \cube{p^{0}_{i}} \) and \(  \Dconstantrelone_{j} = - \Dconstantrelone_{j} \) (since the link capacities are assumed to be symmetric). As demonstrated in Example~\ref{eg:one-shot-control}, \( \Dconstantrelone_{j} \) may contain multiple disjoint intervals that are possibly half open. \qbcomment{Since the objective function in~\eqref{opt:tree-dp-problem} is linear and hence continuous, we assume \( \Dconstantrelone_{j} \) to be closed for all \( j\in \mathcal{E}_{T} \) in this section. } Under constant controls, Proposition~\ref{prop:star-net-invariance} can be recursively applied on the sub-problem  \eqref{opt:tree-dp-value-iteration} as long as the conditions in Proposition~\ref{prop:star-net-invariance} are satisfied. For simplicity, we assume this is indeed the case. As a result, \( \starobj_{i} \) is a \( \roofun \) function for all \( i\in \mathcal{V} \). 
%
%We now introduce some notations. For a real number \( x \), let \( [x]^{+}:= \max\{x, 0\} \)  and \( [x]^{-}:= \min\{x, 0\} \). Hence \( \Dconstantreltwo_{i} = \cube{p_{i}^{0}} = \left[ [p_{i}^{0}]^{-}, [p_{i}^{0}]^{+} \right] \) for all \( i \in \mathcal{V} \). Over domain \( \left[ [p_{i}^{0}]^{-}, [p_{i}^{0}]^{+} \right] \) is a \( \roofun \) function \( \sdsign_{i} y_{i} \) that has top point \( (p_{i}^{0}, |p_{i}^{0}|) \). Let \( q_{i}^{l} : = \min{ \Dconstantrelone } \) and \( q_{i}^{u} : = \max{ \Dconstantrelone } \) for all \( i\in \mathcal{E} \), and let \( \tau_{i} = (\tau_{i}^{1}, \tau_{i}^{2}) \) be the top point and \( [z_{i}^{l}, z_{i}^{u}] := \mathcal{Z}_{i} \) be the domain of function \( g_{i}(z) \) for all \( i\in \mathcal{V} \). One optimal constant load shedding control action is then obtained using the two iteration algorithm, as shown in Algorithm~\ref{alg:two-iterations}. 
Algorithm~\ref{alg:two-iterations} shows the two iterations using two \emph{for} loops. The first loop computes \( \tau_{i} \), \( z_{i}^{l} \) and \( z_{i}^{u} \) for all \( i\in \mathcal{V} \) in reverse topological order according to Lemma~\ref{lem:meta-star-net}, where \( (p_{i}^{0}, |p_{i}^{0}|) \)  on line \ref{alg:top-point-update} is a top point for function \( \sdsign_{i}z_{i} \). The second loop extracts a particular maximizer from the solution set shown in Lemma~\ref{lem:meta-star-net}. 
\begin{remark}
In Algorithm~\ref{alg:two-iterations}, the specific value of \( \gamma_{i} \) is chosen to ensure that the constraint \( z_{i} = u_{i} + \sum_{j\in \mathcal{C}_{i}} z_{i} \) is satisfied. While one can choose other values of \( \gamma_{i} \), this particular choice ensures that the resulting maximizer \( (u_{i}, \{z_{j}\}_{j\in \mathcal{C}_{i}}) \) on lines \ref{alg:sol-extract-1} and \ref{alg:sol-extract-2} to lie in \( \cube{\tau^{1}} \) at every iteration. 
\end{remark}

\begin{example}
Consider the IEEE 39 bus network in Fig.~\ref{fig:ieee39-pic}, with link weights, capacities, and supply-demand vector selected as follows: \( w_{i} = 120 \) for \( i\in \{8, 9\} \), \( w_{i}= 36\) for \( i\in \{11, 12, 15\} \), \( w_{i} = 46 \) for \( i\in \{ 13, 23\} \), \( w_{i} = 24 \) for \( i\in \{ 21, 22\} \), \( w_{i} = 74 \) for \( i\in \{ 18, 19\} \), and \( w_{i} = 80 \) for other links; \( c_{i} = 10 \) for \( i\in \{14, 24, 25, 43, 45\} \), \( c_{i} = 9 \) for \( i\in  \{ 13, 21, 22, 23 \} \), \( c_{i} = 7 \) for \( i\in \{8, 9\} \), \( c_{i} = 3.2 \) for \( i\in \{ 18, 19 \} \), \( c_{i} = 2.5 \) for \( i\in \{ 11, 12, 15\} \), and \( c_{i} =3 \) for other links; \( p_{31} = 10 \), \( p_{6} = -8.5 \), \( p_{16} = -3.5 \), \( p_{19} = -3 \), \( p_{38} = -p_{2} = 2 \), \( p_{17} = 1 \), \( p_{v} = 1 \) for \( v\in \{ 30, 33, 34, 36, 37, 39\} \), and \( p_{v} = 0 \) for other nodes. Consider that a contingency fail links \( 6 \), \( {16} \) and \( {40} \). Then the residual network becomes tree reducible, as shown in Fig.~\ref{fig:def-tree-reducible-net}. With the above parameter, we obtain that \( \Drelone_{2} = [-10, 10] \), \( \Drelone_{7} =[-9.000, -7.987]\cup [-5.326, 5.326]\cup[7.987, 9.000] \) and \( \Drelone_{i} = [0, 3] \) for other links. Table~\ref{tab:ieee-tree-output-fun} shows the results from the two iteration algorithm. It can be seen that, the conditions in Proposition~\ref{prop:star-net-invariance} are satisfied. However, one can verify that the conditions will not be satisfied if link \( 26 \) is also failed by the contingency along with the other three links.
% Requires the booktabs if the memoir class is not being used
\begin{table}[htbp]
   \caption{Output functions for all nodes in Fig.~\ref{fig:reduced-tree}}
   \centering
   %\topcaption{Table captions are better up top} % requires the topcapt package
   \begin{tabular}{lrr} % Column formatting, @{} suppresses leading/trailing space
      \toprule
       & \multicolumn{2}{c}{Output function \( g_{i} \)}  \\  \cmidrule(r){2-3}
            \( i \in \mathcal{V}_{T} \)  &  top point & domain \( Z_{i} \)  \\
      \midrule
      4, 8-12  & \((1, 1)\) & \( [0, 1]\) \\
        5       & \( (2, 2) \)    &  \( [0, 2] \) \\
         7    & \( (10, 10) \)  & \( [0, 10] \) \\
          6   & \( (1, 5) \)  & \( [-2, 3] \) \\
     1  & \( (2, 8) \)   & \( [-3, 5] \) \\
     2  & \( (1.5, 18.5) \) & \( [-8.5, -8]\cup [-5.3, 5.3]\cup [8, 9] \) \\
     3 & \( (-1, 5) \) & \( [-3, 2] \) \\
     4  & \( (1, 1) \)  & \( [0, 1] \) \\
     0  & \( (0, 36) \) & \( [-18, 17] \) \\
      \bottomrule
   \end{tabular}
   \label{tab:ieee-tree-output-fun}
\end{table}

\end{example}

The second condition in Proposition~\ref{prop:star-net-invariance} is related to the relative lengths of the intervals and the gaps between them, and the number sets in summation, as illustrated by Lemma~\ref{lem:sufficient-condition1} and \ref{lem:sufficient-condition2}.  
\begin{lemma}
\label{lem:sufficient-condition1}
Let \( X_{1} \) be a closed interval and \( X_{j} \) be the union of multiple disjoint and closed intervals. Let \( | X_{j}| := \max{X_{j}} - \min{ X_{j}}\) and \( \delta_{j} \) be the maximal length of the gaps between intervals of \( X_{j} \). Assume \( X_{j} \) is labeled such that \( \delta_{j} \le \delta_{j+1} \) for all \( j \), then \( \sum_{j} X_{j} \) is connected if \( \delta_{j+1} \le \sum_{k=1}^{j} |X_{j}| \) for all \( j \).
\end{lemma}
%\begin{remark}
%Lemma~\ref{lem:sufficient-condition1} implies that the second condition in Proposition~\ref{prop:star-net-invariance} is satisfied if \( X_{j} = \real \) for some \( j \in [n] \).
%\end{remark}

\begin{lemma}
\label{lem:sufficient-condition2}
Consider \( m \) disjoint closed intervals denoted by \( X_{j} \), \( j \in [m] \), and labeled in increasing order, that is, \( \max X_{j} < \min X_{j+1} \) for all \( j\in [m-1] \). Let \( |X_{j}| :=  \max{X_{j}} - \min{ X_{j}}\) for all \( j\in [m] \), \( \bar{\delta}_{j} =\min X_{j+1} - \max X_{j}  \) for all \( j\in [m-1] \), and \( X = \cup_{j=1}^{m} X_{j} \). Then  \( \sum_{i=1}^{n} X \) is connected for \( n \ge 1 + \max_{i=1}^{m-1}  {\bar{\delta}_{j}}/ \min\{ |X_{j}|, |X_{j+1}|\} \). 
\end{lemma}
\begin{proof}
We first prove for \( m = 2 \). Let \( X_{1} =: [x_{1}, x_{2}] \) and \( X_{2} =: [x_{3}, x_{4}] \). Then \( \sum_{i=1}^{n} X = \cup_{k= 0}^{n} [(n-k) x_{1} + kx_{3}, (n-k)x_{2}+kx_{4}]  \).
%\begin{equation*}
%\sum_{i=1}^{n} X = \cup_{k= 0}^{n} [(n-k) x_{1} + kx_{3}, (n-k)x_{2}+kx_{4}] 
%\end{equation*}
The necessary and sufficient condition for \( \sum_{i=1}^{n} X  \) to be connected in this case is \((n-k) x_{1} + k x_{3} \le   (n-k+1)x_{2}+(k-1)x_{4}  \) for all \( k \in [n]\), which is equivalent to \( x_{3} - x_{2} \le (n-1) \min\{ x_{2} - x_{1}, x_{4} - x_{3} \} \). The condition can be equivalently written as \( n \ge 1 + \bar{\delta}_{j}/\min\{|X_{1}|, |X_{2}|\} \). Then the assertion for \( m >2 \) follows by considering each adjacent pair of intervals separately. 
\end{proof}


\begin{algorithm}[htb!]
\Input {reduced tree \( \mathcal{T} = ( \mathcal{V}, \mathcal{E}) \), initial supply-demand vector \( p^{0}\in \real^{ \mathcal{V}}\), \( q^{l} \in \real^{ \mathcal{E}} \), \( q^{u} \in \real^{ \mathcal{E}} \)  }
\Output{ optimal constant load shedding control action \( u  \in \real^{ \mathcal{V}} \) }
\For{\( i \in  \mathcal{V} \) in reverse topological order}{
	\( z_{i}^{l}  = \max \left \{q_{i}^{l}, \; [p_{i}^{0}]^{-} + \sum_{j\in \mathcal{C}_{i}} z_{j}^{l} \right \}  \), \( z_{i}^{u}  =\min \left\{ q_{i}^{u}, \; [p_{i}^{0}]^{+} + \sum_{j\in \mathcal{C}_{i}} z_{j}^{u} \right\} \) \; 
	\(  \tau_{i}^{1} = p_{i}^{0} + \sum_{j\in \mathcal{C}_{i}} \tau_{j}^{1}  \), 	\( \tau_{i}^{2} = |p_{i}^{0}| + \sum_{j\in \mathcal{C}_{i}} \tau_{j}^{2}  \) \label{alg:top-point-update} \;
	update \( (\tau_{i}^{1}, \tau_{i}^{2}) \) according to Lemma~\ref{lem:lx-extension} if \( \tau_{i}^{1} \not \in[ q_{i}^{l},  q_{i}^{u}]  \)
}

\( z_{0} = 0 \)\;
\For{\( i \in  \mathcal{V} \) in topological order}{

	\uIf{ \( z_{i} = \tau_{i}^{1} \) }{
		\( u_{i} = p_{i}^{0} \), \( z_{j} =  \tau_{i}^{1} \) for all \( j\in \mathcal{C}_{i} \) \;
	}
	\uElseIf{  \( 0 \le z_{i} < \tau_{i}^{1} \)  }{
	\( \gamma_{i} =\left( z_{i} - \sum_{j\in \mathcal{C}_{i}} [\tau_{j}^{1}]^{-} - [p_{i}^{0}]^{-} \right)/ \left( \sum_{j\in \mathcal{C}_{i}} [\tau_{j}^{1}]^{+} + [p_{i}^{0}]^{+} \right) \)  \;
	\( u_{i} = \min\{p_{i}^{0}, \gamma_{i} p_{i}^{0}\}  \), \(z_{j} = \min \{ \tau_{i}^{1}, \gamma_{i} \tau_{i}^{1} \}\) for all \( j \in \mathcal{C}_{i} \) \label{alg:sol-extract-1} \;
	}\ElseIf{  \( \tau_{i}^{1} < z_{i} < 0  \)  }{
	\( \gamma_{i} =\left( z_{i} - \sum_{j\in \mathcal{C}_{i}} [\tau_{j}^{1}]^{+} - [p_{i}^{0}]^{+} \right)/ \left( \sum_{j\in \mathcal{C}_{i}} [\tau_{j}^{1}]^{-} + [p_{i}^{0}]^{-} \right) \)  \;
	\( u_{i} = \max \{p_{i}^{0}, \gamma_{i} p_{i}^{0}\}  \), \(z_{j} = \max \{ \tau_{i}^{1}, \gamma_{i} \tau_{i}^{1} \}\) for all \( j\in \mathcal{C}_{i} \)  \label{alg:sol-extract-2} \;
	}
}
\Return{\( u \)}
\caption{Optimal constant control for tree reducible network. \label{alg:two-iterations}}
\end{algorithm}

%Given a tree network $  $ with a full dimensional singed supply-demand vector\footnote{Recall the compact supply-demand vector is used in \eqref{eq:power-network-laws} as the zero values are removed.} $ p^{0} \in \real^{ \mathcal{V}}$, its flow solution doesn't depends on link weights and is uniquely determined by the flow conservation equation, that is, \( Af = p^{0} \). This is due to the well known fact that the node-link incidence matrix \( A \)  of a tree is full column rank. Consequently, while removing a zero flow link doesn't affect the flow over the network, removing a nonzero flow link, for example, link failing due to excessive flow, disconnects the network and leads to unbalanced load immediately. Therefore, load shedding has to be applied immediately upon link failure for tree network. Furthermore, a bigger tree network is always capable of supporting greater or equal load than smaller ones. Hence, in response to link failure and in order to support the maximal magnitude of loads, it is not beneficial to apply load shedding over multiple stages for a tree network. To conclude, the optimal load shedding strategy in response to initial link failure over a tree network would be to make it feasible immediately. To compute it, it amounts to solve the LP power redispatch problem \eqref{opt:lp-redispatch} for the tree network. 
%We show how to solve the problem recursively using \eqref{opt:tree-dp-value-iteration}. In this case, \( T = 1 \), for all node \( i\in \mathcal{V} \), \( z_{i} \in \real \) and \( y_{i} = u_{i} \in \real \), \( E_{i} = [-c_{i}, c_{i}] \), \( S_{i} = \cube{p^{0}_{i}} \). For a leaf node \( i \in \mathcal{V} \), it is clear that \( J_{i}(z_{i}) = \sdsign_{i} z_{i} \) for all \( z_{i} \in Z_{i} \). We now consider the problem for first parent \( i\in \mathcal{V} \), where first parent is a node whose children are all leaf nodes. The problem can be equivalently written as: 
%Let  \( \tilde{p}_{v_{1}} := \trans{\onebf} (p^{l} + p^{u}) \) and \( \gamma_{v_{1}} := h_{0}( \bar{\mathcal{C}}_{0}, p) = 2 \min\{\trans{\onebf} p^{u}, -\trans{1} p^{l}\} \), then \(  \trans{\onebf} p^{l} \equiv \frac{1}{2}( \tilde{p}_{v_{1}} - \gamma_{v_{1}} - | \tilde{p}_{v_{1}}| )  \) and \( \trans{\onebf} p^{u} \equiv  \frac{1}{2}( \tilde{p}_{v_{1}} + \gamma_{v_{1}} + | \tilde{p}_{v_{1}}| ) \). 
%For either \( p^{l} = 0 \) or \( p^{u} = 0 \), as \( l(z) = z \) or \( l(z)=-z \), by replacing the redundant variable \( u_{\hat{v}} \) with \( z \) in \( h_{\hat{v}}( \mathcal{E}_{1}, p^{(1)}, z) \), one gets \(  h( \mathcal{E}, p) = h( \mathcal{E}, \tilde{p})  \), where \( \tilde{p}_{ \hat{v}} = \trans{\onebf}{(p^{l}+p^{u})}\) and \( \tilde{p}_{v} = p_{v} \) for all \( v\in \mathcal{V}_{1}\setminus \hat{v} \). In order to get a similar result for the general case \( \trans{\onebf}p^{l} \le 0 \le \trans{\onebf} p^{u} \), we study the following generalized version of \eqref{opt:lp-star} for a star network \( \mathcal{T} = (\mathcal{V}, \mathcal{E}) \). Each leaf \( v \) of the star network incurs an utility \( \roofun_{\tau_{j}}(x_{j}) \) with top point \( x_{v} = ( \trans{\onebf} (p^{u} - p^{l}), \trans{\onebf} (p^{l} + p^{u}) ) \) and domain \( [q_{v}^{l}, q_{v}^{u}] \) and can be seen as the aggregation of a star network rooted at \( v \).

%\eqref{opt:lp-meta-star} is to find a supply-demand \( u \in [q^{l}, q^{u}] \) satisfying \( z = \trans{\onebf} u \) to maximize certain utility over the star network \( (\mathcal{C}_{i} \cup \{i\}, \mathcal{C}_{i}) \). 
%\( l_{j}(u_{j}) \) has domain \( [q_{j}^{l}, q_{j}^{u}] \) and top point \( x_{j} = (x_{j, 1}, x_{j, 2}) \) with \( x_{j, 1} \in [q_{j}^{l}, q_{j}^{u}] \). 

